Long-Term Exploration in Persistent MDPs

Exploration is an essential part of reinforcement learning, which restricts the quality of learned policy. Hard-exploration environments are defined by huge state space and sparse rewards. In such conditions, an exhaustive exploration of the environment is often impossible, and the successful training of an agent requires a lot of interaction steps. In this paper, we propose an exploration method called Rollback-Explore (RbExplore), which utilizes the concept of the persistent Markov decision process, in which agents during training can roll back to visited states. We test our algorithm in the hard-exploration Prince of Persia game, without rewards and domain knowledge. At all used levels of the game, our agent outperforms or shows comparable results with state-of-the-art curiosity methods with knowledge-based intrinsic motivation: ICM and RND. An implementation of RbExplore can be found at https://github.com/cds-mipt/RbExplore.

==> figures/algo-AddTrajectoryToGraph.tex <==
\begin{algorithm}[ht]
\DontPrintSemicolon
\SetKwFunction{FMain}{AddTrajectoryToGraph}
\SetKwProg{Fn}{Function}{:}{}
\KwIn{
\begin{itemize}
    \item $G = (V, E, E_{parent}, count_V, count_E, P)$ --- a weighted directed graph of clusters
    \item $\tau = (s_{1} = \hat{s}, snap_{1} = \hat{snap}), \dots, (s_{T}, snap_{T})$ --- an exploration trajectory starting at the cluster $\hat{v} = (\hat{s}, \hat{snap})$
    \item $R$ --- a similarity model
    \item $\theta_{similarity}$ --- a similarity threshold
\end{itemize}
}
\SetKw{Break}{break}
\Fn{\FMain{$G$, $\tau$, $R$, $\theta_{similarity}$}}{
    $prev\_created\_cluster \leftarrow \hat{v}$, $prev\_visited\_cluster \leftarrow \hat{v}$\;
    $prefix \leftarrow [\ ]$ --- an empty list\; 
    \For{$(s, snap) \in \tau$}{
        $new\_cluster \leftarrow True$\;
        \For{$v = (s_v, snap_v, prefix_v) \in V$}{
            \If{$R(s, s_v) > \theta_{similarity}$}{
                $count_V(s_v) \leftarrow count_V(s_v) + 1$\;
                $count_E((prev\_visited\_cluster, s_v)) \leftarrow count_E((prev\_visited\_cluster, s_v)) + 1$\;
                $prefix \leftarrow prefix + [s]$\;
                $prev\_visited\_cluster \leftarrow v$\;
                $new\_cluster \leftarrow False$\;
                \Break
            }
        }
        \If{$new\_cluster$}{
            $v \leftarrow (s, snap)$\;
            $V \leftarrow V \cup \{v\}$\;
            $E \leftarrow E \cup \{(prev\_visited\_cluster, v)\}$\;
            $arc\_to\_parent \leftarrow (v, prev\_created\_cluster)$
            $E_{parent} \leftarrow E_{parent} \cup \{arc\_to\_parent\}$\;
            $P[arc\_to\_parent] \leftarrow prefix$\;
            $prefix \leftarrow [s]$\;
            $prev\_created\_cluster \leftarrow v$\;
            $prev\_visited\_cluster \leftarrow v$\;
            $\mathbf{continue}$
        }
    }
  }
\caption{AddTrajectoryToGraph}
\end{algorithm}
\label{algo:AddTrajectoryToGraph}

==> figures/algo-RbExplore.tex <==


\begin{algorithm}[ht]
\DontPrintSemicolon
\SetKwFunction{FMain}{RbExplore}
\SetKwProg{Fn}{Function}{:}{}
\KwIn{
\begin{itemize}
    \item $R$ --- a similarity model
    \item $0 \leq \theta_{similarity} \leq 1$ --- a similarity threshold
    \item $\pi_{explore}(a|s)$ --- an exploration policy
    \item $\sigma$ --- a sampling strategy
    \item $RND$ --- a RND module consists of a target and a predictor networks
    \item $\beta_{intrinsic}$ --- an intrinsic reward threshold
    \item $K$ --- maximum allowed number of iterations
\end{itemize}
}    
\KwResult{
$G = (V, E, E_{parent}, count_V, count_E, P)$ --- a weighted directed graph of clusters
\begin{itemize}
    \item $V = \{v_i\} = \{(s_i, snap_i)\}$ --- a set of vertices, $s_i \in \mathcal{S}$ --- a state, $snap_i$ --- a corresponding snapshot of the simulator
    \item $E \subseteq V \times V$ --- a set of arcs
    \item $E_{parent} \subseteq V \times V$ --- a set of arcs to parent clusters
    \item $count_V: V \rightarrow \mathbb{R}$ --- a counter of visits associated to each vertex
    \item $count_E: E \rightarrow \mathbb{R}$ --- a counter of visits associated to each arc
    \item $P$ --- a dictionary storing a set of prefixes to parent clusters for every arc to parent
\end{itemize}
}
\SetKw{AddTrajectoryToGraph}{AddTrajectoryToGraph}
\Fn{\FMain{$R$, $\theta_{similarity}$, $\pi_{explore}$, $\sigma$, $RND$, $\beta_{intrinsic}$, $K$}}{
    $V \leftarrow \{(s_{init}, snap_{init})\}$, $E \leftarrow \emptyset$, $E_{parent} \leftarrow \emptyset$, $count_V \leftarrow \emptyset$, $count_E \leftarrow \emptyset$, $P \leftarrow \emptyset$ \;
    \For{$i \leftarrow 1, \dots, K$}{
    $\{ v_m \}_{m = 1} ^ {M} \sim_{\sigma} G$ --- sample $M$ vertices from $G$\;
    Run exploration with policy $\pi_{explore}$ from the environment's states $\{s_m\}_{m = 1} ^ {M} $ of the selected vertices $\{ v_m \}_{m = 1} ^ {M}$ by restoring the simulator states $\{snap_m\}_{m = 1} ^ {M}$. The result of the exploration is the set of trajectories: $\{\tau_m\}_{m = 1} ^ {M} \leftarrow \{(s_1 ^ m = s_m, snap_1 ^ m = snap_m), \ldots, (s_{T_m}, snap_{T_m})\}$\;
    Create training data set $D$ for the similarity model $R$ from the trajectories $\{\tau_m\}_{m = 1} ^ {M}$\;
    Select all novel states from the trajectories $\{\tau_m\}_{m = 1} ^ {M}$ and place them into a buffer of novel states $B$:
    $B \leftarrow \{\forall (s, snap) \in \{\tau_m\}_{m = 1} ^ {M}: RND(s) > \beta_{intrinsic}\}$\;
    Sample $L$ states from the buffer: $\{(\hat{s}_l, \hat{snap}_l)\}_{l = 1} ^ {L} \sim B$\;
    Run exploration with policy $\pi_{explore}$ from the selected states by restoring the simulator states. The result of the exploration is the set of trajectories: $\{\hat{\tau}_l\}_{l = 1} ^ {L} \leftarrow \{(\hat{s}_1 ^ l = \hat{s}_l, \hat{snap}_1 ^ l= \hat{snap}_l), \ldots, (\hat{s}_{T_l} ^ l, \hat{snap}_{T_l} ^ l)\}$\;
    Create training data set $D$ for the similarity model $R$ from the trajectories $\{\hat{\tau}_l\}_{l = 1} ^ {L}$\;
    $D \leftarrow D \cup \hat{D}$\;
    Train similarity model $R$ on the training data $D$\;
    Train $RND$ on states from $\{\tau_m\}_{m = 1} ^ {M}$\;
    \For{$\tau \in \{\tau_m\}_{m = 1} ^ {M}$}{
        \AddTrajectoryToGraph$(G, \tau, R, \theta_{similarity})$
    }
    \If{$i \bmod merge\_interval = 0$}{
    Merge vertices of $G$\;
    }
    }
    \Return $(V, E, count_V, count_E)$
}
\caption{RbExplore}
\end{algorithm}
\label{algo:RbExplore}
